Datasets, Models, and Algorithms for Multi-Sensor, Multi-agent Autonomy Using AVstack

Recent advancements in assured autonomy have brought autonomous vehicles (AVs) closer to fruition. Despite strong evidence that multi-sensor, multi-agent (MSMA) systems can yield substantial improvements in the safety and security of AVs, there exists no unified framework for developing and testing representative MSMA configurations. Using the recently-released autonomy platform, AVstack, this work proposes a new framework for datasets, models, and algorithms in MSMA autonomy. Instead of releasing a single dataset, we deploy a dataset generation pipeline capable of generating unlimited volumes of ground-truth-labeled MSMA perception data. The data derive from cameras (semantic segmentation, RGB, depth), LiDAR, and radar, and are sourced from ground-vehicles and, for the first time, infrastructure platforms. Pipelining generating labeled MSMA data along with AVstack's third-party integrations defines a model training framework that allows training multi-sensor perception for vehicle and infrastructure applications. We provide the framework and pretrained models open-source. Finally, the dataset and model training pipelines culminate in insightful multi-agent case studies. While previous works used specific ego-centric multi-agent designs, our framework considers the collaborative autonomy space as a network of noisy, time-correlated sensors. Within this environment, we quantify the impact of the network topology and data fusion pipeline on an agent's situational awareness.

==> 5-related-work.tex <==
\section{Related Work} \label{sec:5-related}

\textbf{OPV2V}~\cite{2022openv2v}, the Open Dataset for Perception with V2V communication, provided one of the first labeled datasets with multi-agent perception sensing data. OPV2V logs LiDAR point clouds from between 3-7 agents from the \carla\ simulator. These point clouds are used to perform a trade study of data fusion techniques. While OPV2V is a useful starting point for multi-agent autonomy, it cannot be a \textit{general} framework for multi-agent autonomy due to its primitive reference frame transformations, lack of support for infrastructure sensing, and limited, specialized perception models that are specially designed for their datasets alone.

% \textbf{ROS}~\cite{2009ros} provides a communication infrastructure above operating systems for multi-component robotics applications. ROS handles message passing between peer nodes in full-stack robotics case studies. In this way, ROS has greatly streamlined the development process for deployable robotics and has been recognized as a major research platform.

% \textbf{Pylot}~\cite{2021pylot} is an AV architecture in the Python language. Sensor data is passed using the low-latency, low-copy ERDOS~\cite{2021pylot} framework. Pylot provides an accessible interface where developers can compare algorithms within established components on the CARLA simulator~\cite{2017carla}. Pylot demonstrated near-real-time capability on a real system at low speeds. While Pylot maintains an accessible API, it is limited to the CARLA simulator and real-world self-driving; it cannot be tested on benchmark datasets. While it supports different algorithms within each component, the component architecture is fixed. It is not suitable for next-level questions such as multi-agent, collaborative sensing nor does it support end-to-end learning-based implementations.


==> tables/scenario-variables.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%          TODO & TODO  \\
%          & 
%     \end{tabular}
%     \caption{Available scenario parameters for unique generation of diverse labeled datasets from integration of \carla\ with \avstack.}
%     \label{tab:scenario-variables}
% \end{table}
